Deep Learning from Shallow Dives: Sonar Image Generation and Training for Underwater Object Detection

Among underwater perceptual sensors, imaging sonar has been highlighted for its perceptual robustness underwater. The major challenge of imaging sonar, however, arises from the difficulty in defining visual features despite limited resolution and high noise levels. Recent developments in deep learning provide a powerful solution for computer-vision researches using optical images. Unfortunately, deep learning-based approaches are not well established for imaging sonars, mainly due to the scant data in the training phase. Unlike the abundant publically available terrestrial images, obtaining underwater images is often costly, and securing enough underwater images for training is not straightforward. To tackle this issue, this paper presents a solution to this field's lack of data by introducing a novel end-to-end image-synthesizing method in the training image preparation phase. The proposed method present image synthesizing scheme to the images captured by an underwater simulator. Our synthetic images are based on the sonar imaging models and noisy characteristics to represent the real data obtained from the sea. We validate the proposed scheme by training using a simulator and by testing the simulated images with real underwater sonar images obtained from a water tank and the sea.

==> fig_sample.tex <==
\begin{figure*}[!t]
  \centering
  \subfigure[Sample 1]{%
    \includegraphics[width = 0.89\columnwidth]{figs/CKI_BD.jpg}
    \label{CKIBD}
  }
  \subfigure[Sample 2]{%
    \includegraphics[width = 0.9\columnwidth]{figs/CKI_NB.jpg}
    \label{CKINB}
  }\\
  %\subfigure[Sample image with body \texttt{TDI-BD}]{%
  %  \includegraphics[width = 0.9\columnwidth]{figs/TDI_BD.jpg}
  %  \label{TDIBD}
  %}
  %\subfigure[Sample image without body \texttt{TDI-NB}]{%
  %  \includegraphics[width = 0.9\columnwidth]{figs/TDI_NB.jpg}
  %  \label{TDINB}
  %}

    \caption{Style tranfer performance. Sample images are synthesized from the
    simulator-generated images by style tranfer.}

  \label{fig:style_results}
\end{figure*}


==> fig_synth.tex <==
%FIGURE
\renewcommand*{\thesubfigure}{}
\begin{figure*}[!t]
  \centering
  \def\width{0.3\columnwidth}%

  \begin{minipage}{0.47\textwidth}%
  \centering
  Images with the target object (\texttt{BD})
  \subfigure{
    \includegraphics[width=0.05\textwidth]{figs/cki_txt}
    \includegraphics[width=\width]{figs/synth/cki_resize_and_crop_BD.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_rotation_BD.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_translation_BD.jpg}
  }
  %---------------------------------------------------------------------%
  \subfigure{
    \includegraphics[width=0.05\textwidth]{figs/cki_fft_txt}
    \includegraphics[width=\width]{figs/synth/cki_fft_resize_and_crop_BD.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_fft_rotation_BD.jpg}
  }%
  \subfigure{    
    \includegraphics[width=\width]{figs/synth/cki_fft_translation_BD.jpg}
  }
  %---------------------------------------------------------------------%
  \subfigure{  
    \includegraphics[width=0.05\textwidth]{figs/cki_style_txt}
    \includegraphics[width=\width]{figs/synth/cki_style_resize_and_crop_BD.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_style_rotation_BD.jpg}
  }%
  \subfigure{    
    \includegraphics[width=\width]{figs/synth/cki_style_translation_BD.jpg}
  }
  %---------------------------------------------------------------------%
  \subfigure[Scale and crop]{  
    \includegraphics[width=0.05\textwidth]{figs/tdi_txt}
    \includegraphics[width=\width]{figs/synth/tdi_resize_and_crop_BD.jpg}
  }%
  \subfigure[Rotation]{    
    \includegraphics[width=\width]{figs/synth/tdi_rotation_BD.jpg}
  }%
  \subfigure[Translation]{
    \includegraphics[width=\width]{figs/synth/tdi_translation_BD.jpg}
  }
  \end{minipage}
  %---------------------------------------------------------------------%
  \hfill
  %---------------------------------------------------------------------%
  \begin{minipage}{0.495\textwidth}%
  \centering
  Images without the target object (\texttt{NB})
  \subfigure{    
    \includegraphics[width=\width]{figs/synth/cki_resize_and_crop_NB.jpg}
  }%
  \subfigure{    
    \includegraphics[width=\width]{figs/synth/cki_rotation_NB.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_translation_NB.jpg}
  }
  %---------------------------------------------------------------------%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_fft_resize_and_crop_NB.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_fft_rotation_NB.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_fft_translation_NB.jpg}
  }
  %---------------------------------------------------------------------%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_style_resize_and_crop_NB.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_style_rotation_NB.jpg}
  }%
  \subfigure{
    \includegraphics[width=\width]{figs/synth/cki_style_translation_NB.jpg}
  }    
  %---------------------------------------------------------------------%
  \subfigure[Scale and crop]{
    \includegraphics[width=\width]{figs/synth/tdi_resize_and_crop_NB.jpg}
  }%
  \subfigure[Rotation]{    
    \includegraphics[width=\width]{figs/synth/tdi_rotation_NB.jpg}
  }%
  \subfigure[Translation]{    
    \includegraphics[width=\width]{figs/synth/tdi_translation_NB.jpg}
  }    
  \end{minipage}%

  \caption{From the top row, sample images from \texttt{CKI}, \ac{FFT} applied
  \texttt{CKI}, style transferred \texttt{CKI}, and \texttt{TDI}. When
  generating images we applied scale, crop, rotation, and translational
  variation.}

  \label{fig:img_train}
\end{figure*}
\renewcommand*{\thesubfigure}{(\alph{subfigure})}
%FIGURE

